Understanding Routing-Induced Censorship Changes Globally

Internet censorship is pervasive, with significant effort dedicated to understanding what is censored, and where. Prior censorship work however have identified significant inconsistencies in their results; experiments show unexplained non-determinism thought to be caused by censor load, end-host geographic diversity, or incomplete censorship -- inconsistencies which impede reliable, repeatable and correct understanding of global censorship. In this work we investigate the extent to which Equal-cost Multi-path (ECMP) routing is the cause for these inconsistencies, developing methods to measure and compensate for them. We find ECMP routing significantly changes observed censorship across protocols, censor mechanisms, and in 17 countries. We identify that previously observed non-determinism or regional variations are attributable to measurements between fixed end-hosts taking different routes based on Flow-ID; i.e., choice of intra-subnet source IP or ephemeral source port leads to differences in observed censorship. To achieve this we develop new route-stable censorship measurement methods that allow consistent measurement of DNS, HTTP, and HTTPS censorship. We find ECMP routing yields censorship changes across 42% of IPs and 51% of ASes, but that impact is not uniform. We identify numerous causes of the behavior, ranging from likely failed infrastructure, to routes to the same end-host taking geographically diverse paths which experience differences in censorship en-route. Finally, we explore our results in the context of prior global measurement studies, exploring first the applicability of our findings to prior observed variations, and then demonstrating how specific experiments from two studies could be impacted by, and specific results are explainable by, ECMP routing. Our work points to methods for improving future studies, reducing inconsistencies and increasing repeatability.

==> Makefile <==
#
# Updated Makefile, trimmed from:
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PAPER = apppaths
INCLUDES = figs

# Setting up a new paper, you should be able to grab this file and not edit below this line

all:  $(PAPER).pdf

once: *.tex $(INCLUDES)* *.bib Makefile 
	pdflatex $(PAPER)

$(PAPER).pdf: *.tex $(INCLUDES)* *.bib Makefile   
	pdflatex $(PAPER)
	- bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(PAPER).log) \
	do pdflatex $(PAPER); done


.PHONY: clean

clean:
	$(RM) $(PAPER).pdf diff.pdf *.log *.aux \
	abstract.txt *.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi


